Self-supervision meets kernel graph neural models: From architecture to augmentations

Graph representation learning has now become the de facto standard when handling graph-structured data, with the framework of message-passing graph neural networks (MPNN) being the most prevailing algorithmic tool. Despite its popularity, the family of MPNNs suffers from several drawbacks such as transparency and expressivity. Recently, the idea of designing neural models on graphs using the theory of graph kernels has emerged as a more transparent as well as sometimes more expressive alternative to MPNNs known as kernel graph neural networks (KGNNs). Developments on KGNNs are currently a nascent field of research, leaving several challenges from algorithmic design and adaptation to other learning paradigms such as self-supervised learning. In this paper, we improve the design and learning of KGNNs. Firstly, we extend the algorithmic formulation of KGNNs by allowing a more flexible graph-level similarity definition that encompasses former proposals like random walk graph kernel, as well as providing a smoother optimization objective that alleviates the need of introducing combinatorial learning procedures. Secondly, we enhance KGNNs through the lens of self-supervision via developing a novel structure-preserving graph data augmentation method called latent graph augmentation (LGA). Finally, we perform extensive empirical evaluations to demonstrate the efficacy of our proposed mechanisms. Experimental results over benchmark datasets suggest that our proposed model achieves competitive performance that is comparable to or sometimes outperforming state-of-the-art graph representation learning frameworks with or without self-supervision on graph classification tasks. Comparisons against other previously established graph data augmentation methods verify that the proposed LGA augmentation scheme captures better semantics of graph-level invariance.

==> tables/datasets.tex <==
\begin{tabular}{lcccccccc}
    \toprule
     & MUTAG & D\&D & NCI1 & PROTEINS & IMDB-B & COLLAB & RDT-B & RDT-M5K \\
    \midrule
    \# graphs & $188$ & $1178$ & $4110$ & $1113$ & $1000$ & $5000$ & $2000$ & $4999$ \\
    \# classes & $2$ & $2$ & $2$ & $2$ & $2$ & $3$ & $2$ & $5$ \\
    % \# node features & \na & \na & \na & $1$ & \na & \na & \na & \na \\
    \# node features & 7 & 82 & 37 & 3 & \na & \na & \na & \na \\
    Average \# nodes & $17.93$ & $284.32$ & $29.87$ & $39.05$ & $19.77$ & $74.49$ & $429.61$ & $508.50$ \\
    Average \# edges & $19.79$ & $715.66$ & $32.30$ & $72.81$ & $96.53$ & $2457.34$ & $497.75$ & $594.87$ \\
    \bottomrule
\end{tabular}

==> tables/peformance_full.tex <==
\begin{tabular}{lccccccccc}
    \toprule
     & MUTAG & D\&D & NC1 & PROTEINS & IMDB-B & IMDB-M & COLLAB & RDT-B & RDT-M5K 
   \\
   \midrule
   SP & \result{80.2}{6.5} & \result{78.1}{4.1} & \result{72.7}{1.4} & \result{75.3}{3.8} & \result{57.7}{4.1} & \result{39.8}{3.7} & \result{79.9}{2.7} & \result{89.0}{1.0} & \result{51.1}{2.2}
   \\
   GR & \result{80.8}{6.4} & \result{75.4}{3.4} & \result{61.8}{1.7} & \result{71.6}{3.1} & \result{63.3}{2.7} & \result{39.6}{3.0} & \result{71.1}{1.4} & \result{76.6}{3.3} & \result{38.1}{2.3}
   \\
   WL & \result{84.6}{8.3} & \result{78.1}{2.4} & \result{84.8}{2.5} & \result{73.8}{4.4} & \result{72.8}{4.5} & \result{51.2}{6.5} & \result{78.0}{2.0} & \result{74.9}{1.8} & \result{49.6}{2.0}
   \\
   \midrule
   DGCNN & \result{84.0}{6.7} & \result{76.6}{4.3} & \result{76.4}{1.7} & \result{72.9}{3.5} & \result{69.2}{3.0} & \result{45.6}{3.4} & \result{71.2}{1.9} & \result{87.8}{2.5} & \result{49.2}{1.2}
   \\
   DiffPool & \result{79.8}{7.1} & \result{75.0}{3.5} & \result{76.9}{1.9} & \result{73.7}{3.5} & \result{68.4}{3.3} & \result{45.6}{3.4} & \result{68.9}{2.0} & \result{89.1}{1.6} & \result{53.8}{1.4}
   \\
   GIN & \result{84.7}{6.7} & \result{75.3}{2.9} & \result{80.0}{1.4} & \result{73.3}{4.0} &\result{71.2}{3.9} & \result{48.5}{3.3} & \result{75.6}{2.3} & \result{89.9}{1.9} & \result{56.1}{1.7}
   \\
   GraphSAGE & \result{83.6}{9.6} & \result{72.9}{2.0} & \result{76.0}{1.8} & \result{73.0}{4.5} & \result{68.8}{4.5} & \result{47.6}{3.5} & \result{73.9}{1.7} & \result{84.3}{1.9} & \result{50.0}{1.3}
   \\
   \midrule
   InfoGraph(paper) & \result{87.7}{1.8} & \result{75.2}{0.39} & \result{68.1}{0.59} & \result{72.6}{0.7} & \result{71.1}{0.9} & \result{48.7}{0.7} & \result{70.4}{0.6} & \result{78.8}{2.1} & \result{51.1}{0.6}
   \\
   GraphCL(paper) & \result{88.3}{1.3} & \result{74.7}{0.7} & \result{68.5}{0.6} & \result{72.9}{1.0} & \result{70.8}{0.8} & \result{48.5}{0.6} & \result{71.3}{0.6} & \result{82.6}{1.0} & \result{53.1}{0.4}
   \\
   AD-GCL(paper) & \result{89.3}{1.5} & \result{74.5}{0.5} & \result{69.7}{0.5} & \result{73.6}{0.7} & \result{71.6}{1.0} & \result{49.0}{0.5} & \result{73.3}{0.6} & \result{85.5}{0.8} & \result{53.0}{0.8}
   \\
   RGCL(paper) & \result{87.7}{1.0} & \result{78.9}{0.5} & \result{78.1}{1.1} & \result{75.0}{0.4} & \result{71.9}{0.8} & \result{}{} & \result{70.9}{0.7} & \result{90.3}{0.6} & \result{56.4}{0.4}
   \\
   GCL-SPAN(paper) & \result{89.1}{0.8} & \result{75.8}{0.5} & \result{71.4}{0.5} & \result{75.8}{0.4} & \result{73.7}{0.7} & \result{52.2}{0.7} & \result{75.0}{0.5} & \result{83.6}{0.6} & \result{54.1}{0.5}
   \\
   GraphMAE(paper) & \result{88.2}{1.3} & \result{}{} & \result{80.4}{0.3} & \result{75.3}{0.4} & \result{75.5}{0.7} & \result{51.6}{0.5} & \result{80.3}{0.5} & \result{88.0}{0.2} & \result{}{} \\
   \midrule
   GraphMAE(rerun) & \result{85.6}{1.4} & \result{72.9}{1.6} & \result{79.3}{0.5} & \result{75.7}{0.3} & \result{75.4}{0.6} & \result{50.2}{0.6} & \result{80.2}{0.2} & \result{84.5}{0.5} & \result{52.9}{0.3}
   \\
   RGCL(rerun) & \result{89.9}{6.2} & \result{78.8}{3.2} & \result{78.4}{2.1} & \result{75.5}{3.8} & \result{73.2}{4.0} & \result{49.8}{2.4} & \result{70.8}{1.7} & \result{89.5}{2.5} & \result{56.2}{2.1} \\
   AD-GCL(rerun) & \result{88.1}{1.4} & \result{7e.8}{0.7} & \result{69.4}{0.6} & \result{73.6}{0.6} & \result{71.2}{0.5} & \result{48.4}{0.9} & \result{73.3}{0.5} & \result{84.9}{1.4} & \result{54.9}{0.7} \\
   GCC(rerun) & \result{83.6}{7.4} & \result{67.9}{2.3} & \result{68.0}{2.0} & \result{67.2}{2.4} & \result{74.4}{4.0} & \result{49.5}{3.2} & \result{77.5}{1.7} & \result{85.5}{3.1} & \result{48.7}{1.2} \\
   InfoGraph(rerun) & \result{87.7}{6.7} & \result{79.5}{2.1} & \result{80.3}{1.8} & \result{74.1}{3.6} & \result{71.4}{2.9} & \result{48.5}{3.8} & \result{75.4}{2.1} & \result{91.1}{1.5} & \result{56.5}{1.2} \\
   GCL-SPAN(rerun) & \result{83.5}{6.5} & \result{77.8}{3.5} & \result{69.8}{2.0} & \result{73.0}{3.5} & \result{71.5}{3.1} &  & \result{66.0}{1.2} & \result{71.9}{3.0} & \result{36.1}{2.2} \\
   GCL-SPAN(rerun2) & \result{85.7}{7.9} & \result{79.5}{3.2} & \result{76.9}{2.0} & \result{74.2}{4.4} & \result{76.2}{3.0} & \result{}{} & \result{71.3}{2.0} & \result{84.2}{2.0} & \result{53.7}{1.7} \\
   GraphCL(rerun) & \result{81.5}{7.0} & \result{70.4}{3.8} & \result{72.4}{3.0} & \result{69.3}{3.6} & \result{64.7}{5.1} & \result{}{} & \result{74.4}{1.3} & \result{83.4}{3.0} & \result{49.9}{1.3} \\
   \midrule
   RGCL(rwgnn) & \result{83.5}{8.3} & \result{74.8}{3.8} & \result{64.2}{2.1} & \result{72.7}{2.6} & \result{70.9}{3.9} & \result{46.7}{2.3} & \result{68.2}{2.4} & \result{82.9}{2.7} & \result{49.5}{1.9} \\
   GCC(rwgnn) & \result{84.7}{6.7} & \result{74.9}{4.8} & \result{67.0}{1.9} & \result{72.1}{3.0} & \result{71.1}{4.7} & \result{48.9}{2.5} & \result{78.3}{1.6} & \result{85.1}{2.8} & \result{49.0}{1.1} \\
   GCL-SPAN(rwgnn) & \result{85.2}{8.5} & \result{76.2}{2.8} & \result{62.6}{2.7} & \result{75.2}{4.5} & \result{71.4}{2.7} & & \result{68.4}{1.9} & \result{79.4}{1.9} & \result{49.0}{2.3} \\
   GraphCL(rwgnn) & \result{86.2}{6.3} & \result{75.1}{3.0} & \result{67.7}{2.8} & \result{71.0}{4.5} & \result{67.7}{4.4} & & \result{73.1}{1.8} & \result{82.1}{4.9} & \result{52.9}{2.1} \\
    \midrule
   RWGNN    & \result{89.2}{4.3} & \result{77.6}{4.7} & \result{73.9}{1.3} & \result{74.7}{3.3} & \result{70.6}{4.4} & \result{48.8}{2.9} & \result{71.9}{2.5} & \result{90.4}{1.9} & \result{53.4}{1.6}
   \\
   \midrule
   SWAG     & \result{89.4}{6.0} & \result{76.6}{5.0} & \result{70.2}{2.2} & \result{76.3}{4.4} & \result{73.1}{3.3} & \result{43.0}{4.8} & \result{74.1}{1.6} & \result{90.3}{1.8} & \result{55.4}{2.2} 
   \\
   SWAG+LGA(infonce) & \result{89.1}{6.7} & \result{76.3}{5.0} & \result{70.7}{1.9} & \result{76.3}{4.3} & \result{74.0}{2.9} & \result{43.5}{5.2} & \result{74.6}{2.5} & \result{91.5}{1.7} & \result{56.0}{2.1}
   \\
   SWAG+LGA(simsiam) & \result{90.3}{6.2} & \result{77.5}{4.4} & \result{70.9}{2.4} & \result{77.5}{4.5} & \result{74.4}{3.3} & \result{43.5}{4.4} & \result{74.1}{2.0} & \result{91.5}{1.7} & \result{56.0}{2.1} 
   \\
   \bottomrule
\end{tabular}

==> tables/performance_reduced.tex <==
\begin{tabular}{lccccccccc}
    \toprule
     & MUTAG & D\&D & NC1 & PROTEINS & IMDB-B & IMDB-M & COLLAB & RDT-B & RDT-M5K \\
    \midrule
   RWGNN    & \result{85.5}{9.0} & \result{76.7}{5.0} & \result{67.3}{1.4} & \result{74.6}{4.4} & \result{73.4}{3.8} & \result{43.0}{6.3} & \result{71.9}{2.5} & \result{87.1}{4.2} & \result{54.0}{2.5} \\
   \midrule
   SWAG     & \result{87.8}{7.7} & \result{76.3}{4.5} & \result{69.0}{1.5} & \result{74.9}{4.9} & \result{69.8}{5.2} & \result{42.3}{5.7} & \result{71.6}{2.4} & \result{87.5}{2.9} & \result{55.1}{1.4} \\
   SWAG+LGA & \result{88.8}{8.4} & \result{76.4}{4.1} & \result{69.3}{2.0} & \result{75.2}{5.3} & \result{72.0}{4.0} & \result{43.3}{4.3} & \result{71.9}{1.9} & \result{89.5}{2.5} & \result{54.6}{2.0} \\
   \bottomrule
\end{tabular}
